Measuring large-scale social networks with high resolution

This paper describes the deployment of a large-scale study designed to measure human interactions across a variety of communication channels, with high temporal resolution and spanning multiple years - the Copenhagen Networks Study. Specifically, we collect data on face-to-face interactions, telecommunication, social networks, location, and background information (personality, demographic, health, politics) for a densely connected population of 1,000 individuals, using state-of-art smartphones as social sensors. Here we provide an overview of the related work and describe the motivation and research agenda driving the study. Additionally the paper details the data-types measured, and the technical infrastructure in terms of both backend and phone software, as well as an outline of the deployment procedures. We document the participant privacy procedures and their underlying principles. The paper is concluded with early results from data analysis, illustrating the importance of multi-channel high-resolution approach to data collection.

==> sections/figure_legends.tex <==
\section{Figure Legends}

%\begin{figure}[!ht]
%\begin{center}
%	\includegraphics[width=1\textwidth]{fig_authorizations}
%\end{center}
%\caption{
%{\bf Authorizations page.} Participants have an overview of the studies they are enrolled into and application that can submit and access their data. This is an important step towards user's understanding of what is happening with their data and to exercise control over it.}
%\label{fig:authorizations}
%\end{figure}

%\begin{figure}[!ht]
%\begin{center}
%	\includegraphics[width=1\textwidth]{fig_data_viewer}
%\end{center}
%\caption{
%{\bf Data viewer application.} All the collected data can be explored and access via an API. The API is the same for research, application, and end-user access, the endpoints are OAuth2 bearer token protected.}
%\label{fig:fig_data_viewer}
%\end{figure}

%\begin{figure}[!ht]
%\begin{center}
%	\includegraphics[width=1\textwidth]{fig_openpdsarch}
%\end{center}
%\caption{
%{\bf Sensible Data open Personal Data System architecture.} This system was used in 2013 deployment and consists of three layers: platform, services, and applications. Platform contains element common for multiple services (in this context: studies). Studies are the deployments of particular data collection efforts. Applications are OAuth2 clients to studies and can submit and access data, based on user authorizations.}
%\label{fig:openpdsarch}
%\end{figure}

% \begin{figure}[!ht]
% \begin{center}
% 	\includegraphics[width=1\textwidth]{fig_group.pdf}
% \end{center}
% \caption{
% {\bf Group dynamics.} The evolution of a group, as observed from the perspective of node $126$. For each time-window a link is draw if either person $i \rightarrow j$ or $i \leftarrow j$. }
% \label{fig:dynamics}
% \end{figure}





